MMTM: Multimodal Transfer Module for CNN Fusion

In late fusion, each modality is processed in a separate unimodal Convolutional Neural Network (CNN) stream and the scores of each modality are fused at the end. Due to its simplicity late fusion is still the predominant approach in many state-of-the-art multimodal applications. In this paper, we present a simple neural network module for leveraging the knowledge from multiple modalities in convolutional neural networks. The propose unit, named Multimodal Transfer Module (MMTM), can be added at different levels of the feature hierarchy, enabling slow modality fusion. Using squeeze and excitation operations, MMTM utilizes the knowledge of multiple modalities to recalibrate the channel-wise features in each CNN stream. Despite other intermediate fusion methods, the proposed module could be used for feature modality fusion in convolution layers with different spatial dimensions. Another advantage of the proposed method is that it could be added among unimodal branches with minimum changes in the their network architectures, allowing each branch to be initialized with existing pretrained weights. Experimental results show that our framework improves the recognition accuracy of well-known multimodal networks. We demonstrate state-of-the-art or competitive performance on four datasets that span the task domains of dynamic hand gesture recognition, speech enhancement, and action recognition with RGB and body joints.

==> AVSE_sections/01_AVSE_related_works.tex <==

% \subsection{Audio-Visual Speech Enhancement}
% \mli{TEMPORARY: Taken verbatim from ICASSP. Needs rephrasing / editing. Feel free to change/delete anything below as is necessary for better fit.}

% Work in audio-visual speech enhancement (AVSE) is strongly motivated by the cocktail party effect, which refers to humans' ability to selectively attend to auditory signals of interest within a noisy environment. Research on the subject dates back to attention experiments conducted by Colin Cherry in 1953 \cite{cherry1953some}. Experiments in neuroscience have demonstrated that cross-modal integration of audio-visual signals may improve the perceptual quality of the targeted acoustic signal \cite{ghazanfar2003neuroperception, partan1999communication, rowe2002sound}. Psycho-linguistic studies have investigated the effects of visual information on auditory encoding: \cite{moradi2013gated} showed that visual cues speed up linguistic recognition under noisy listening conditions, and \cite{stenzel2019limits} demonstrated that spatial decoherence between audio and visual sources affect percept encoding. 

% Historically, the field of signal processing focused on audio-only (AO) approaches to speech enhancement. Inspired by the results from biological research, the field has shifted to augmenting these approaches with visual information, such as lip movement. State-of-the-art results have been achieved by recent AV speech enhancement models that use deep neural networks \cite{afouras2018conversation, ephrat2018looking, afouras2019my, hou2018audio}. The predominant approach taken for AV fusion is late fusion \cite{katsaggelos2015audiovisual}, where the audio and visual information is processed separately then integrated at a singular point via channel-wise concatenation. These approaches have achieved some degree of a computational cocktail party effect, but late fusion does not allow for feature-level correlation across modalities, and relatively minimal work has explored alternative mechanisms to channel-wise feature concatenation for cross-modal integration.

% In computer vision, one of the first works on video classification using deep neural networks compared late fusion, slow fusion, and early fusion of time-based, uni-modal visual signals \cite{karpathy2014large}. This work demonstrated that slow fusion was most effective, motivating our exploration of slow fusion methods for AV integration. Further, channel-wise concatenation of cross-modal signals is commonly used for conditional generative models. Yet a recent study shows that concatenation of cross-modal information does not effectively model the underlying correlations between features \cite{miyato2018cgans}. Squeeze-excitation (SE) networks \cite{hu2018squeeze} offer an alternative to channel-wise concatenation via a light-weight, adaptive gating mechanism that has been demonstrated to work well on sound event detection \cite{xia2019sound}.

% In this work, we explore alternative approaches to audio-visual (AV) fusion within a deep learning framework and propose an improved method and mechanism. We propose a squeeze-excitation (SE) fusion block that integrates AV information across multiple levels of audio and visual feature representations within both late and slow fusion schemes. We generate visual features according to \cite{stafylakis2017combining}, and following \cite{gabbay2017visual, michelsanti2019training} we use an autoencoder neural network with skip connections as our audio network. However, our approach differs from the findings of \cite{michelsanti2019training} on optimal target domains, and we train our objective using the indirect mapping approach of \cite{afouras2018conversation, ephrat2018looking} with log-mel transformed inputs. We compare our method, AV(SE)$^2$, against the late fusion methods for AV speech enhancement and demonstrate that the SE fusion block yields improvements in performance and up to a 37\% reduction in the number of model parameters.

==> AVSE_sections/02_AVSE_experiments.tex <==
% \label{sec:av_experiment}
% \mlic{Ensure sentence is included referencing Zisserman results and why there are no direct comparisons in the audio domain.}
% In this section, we evaluate our MMTM method on audio-visual speech enhancement (AVSE). Using PESQ and STOI objective measures, we demonstrate that our slow fusion MMTM method outperforms state-of-the-art late fusion, channel-wise concatenation AVSE approaches.

% We use \textit{VoxCeleb2} \cite{chung2018voxceleb2}, a large audio-visual dataset obtained from YouTube that contains over 1 million utterances for 6,112 celebrities. The training, validation, and test datasets are split by celebrity ID (CID) such that the sets are disjoint over CIDs. In addition, CHiME-1/3 \cite{barker2013csl,Barker2017csl}, NonStationaryNoise \cite{duan2012online}, ESC50 \cite{piczak2015dataset}, HuCorpus \cite{hu2010tandem}, and private datasets are used for additive noise.

% Video frames are extracted at 25 FPS and S$^3$FD \cite{zhang2017s3fd} performs face detection. Following \cite{stafylakis2017combining}, we discard redundant visual information by cropping the mouth region via facial landmarks obtained from Facial Alignment Network \cite{bulat2017far}. Lip frames are resized to $122 \times 122$, transformed to grayscale, then normalized using the global mean and variance statistics from the training set. The audio waveform is extracted from the video following the methods of \cite{afouras2018conversation, gabbay2017visual}. We specify a window length of 40ms, hop size of 10ms, and sampling rate of 16kHz to align one video frame to four audio steps. Short-time Fourier transform (STFT) with a Hanning window function converts the waveform to spectrogram, $X_{spec} \in \mathbb{R}^{T \times F}$ with a frequency resolution of $F=321$, representing frequencies from $0-8$kHz. 

% Training samples are generated on-the-fly as lip frame and spectrograms pairs, ($X_{vid}, X_{spec}$), with a batch size of 4. A interference spectrogram, $X_{inter}$, is randomly sampled from the VoxCeleb2 set, and  noise spectrogram, $X_{n}$, is randomly sampled from the noise datasets. The mixture signal, $X_{mix}$, is obtained as $X_{mix} = X_{spec} + \alpha X_{inter} + \beta X_{n}$, where $\alpha, \beta$ are mixing coefficients computed to achieve a specific SNR value. Training and test SNR values are randomly sampled from the range of 0-20dB and 2.5-17.5dB, respectively. $X_{mix}$ is transformed to a log-mel representation, $\log X_{mel} \in \mathbb{R}^{T \times F}$, where $T=116$ and $F=80$. We augment lip frames, $X_{vid}$, via random cropping ($\pm$ 5 pixels) and left-right flips. Augmented frames are resized to $112 \times 112$ and fed into the visual network. 


% %\subsubsection{Implementation Details} 

% % Experiment Results
% \input{AVSE_sections/tables/AV_results.tex}


% %%% RESULTS
% % --------------------------------------------------
% Objective evaluation results are shown in Table \ref{table:AVSE_results}. We evaluate enhanced speech using the perceptual quality of speech quality (PESQ) \cite{recommendation2001perceptual}, an objective measure of subjective listening tests, and the short-time objective intelligibility (STOI) \cite{taal2011algorithm}, which is highly correlated with the intelligibility of noisy speech. The audio only (AO) model is trained without the visual network and establishes an AO speech enhancement baseline. The AV baseline model establishes a baseline for the predominant AVSE approaches that perform late-fusion via channel-wise concatenation (CWC) of AV features. Our v1 model performs late fusion, but replaces the CWC fusion mechanism with our MMTM. Lastly, Our v2 model applies MMTM across multiple AV feature levels to demonstrate our full slow fusion MMTM approach. 

% Our v1 outperforms the AO and AV baselines, demonstrating that MMTM provides an optimal fusion mechanism compared to CWC. Our v2 model achieves the best PESQ and STOI measures, outperforming the AO and AV baselines as well as our v1 model. This indicates that MMTM via slow fusion affords the greatest performance improvements. Further, the AV baseline has $\sim$54 million (M) parameters, but our v2 model has $\sim$34M, a 35\% reduction. Our model generalizes to speakers unseen during training since CID is disjoint across train and test sets.
% % --------------------------------------------------------




==> AVSE_sections/tables/AV_results.tex <==
% % Nice table reference: https://inf.ethz.ch/personal/markusp/teaching/guides/guide-tables.pdf

% \begin{table}[tp]
%     \small \centering
% \begin{tabular}{lccc} %\toprule 
% Method & Fusion & PESQ & STOI \\
% \midrule
% Target & - & 4.64 & 1.000 \\
% Mixed  & - & 2.19 & 0.900 \\
% \hline
% % AVSE (CWC) \cite{afouras2018conversation} & 2.59 & 0.65 
% AO Baseline & - & 2.43 & 0.930\\
% AV Baseline & CWC & 2.67 & 0.938\\
% % Bottleneck
				
% Ours & MMTM-4 & 2.73 & \best{0.941} \\
% Ours & MMTM-3 & 2.74 & 0.939 \\
% Ours & MMTM-2 & 2.70 & 0.938 \\
% Ours & MMTM-1 & \best{2.79} & 0.940 \\
% \hline\hline
% %\bottomrule
% \end{tabular}
% \caption{\mlic{These are the most recent evaluations on 3 simultaneous speakers. However, the table needs to be adjusted such that it matches the paper. I put in all information, but please adjust to best fit.}Speech enhancement evaluations on the VoxCeleb2 dataset \cite{chung2018voxceleb2} for 3 simultaneous speakers. CWC: Channel-wise concatenation. The best performance is denoted by boldface.}
% \label{table:AVSE_results}
% \vspace{-0.2in}
% \end{table}

==> backups/section_2.tex <==
In general, multimodal fusion can be achieved at the feature level (i.e. early fusion), decision level (i.e. late fusion) or intermediately~\cite{ramachandram2017deep}. In late fusion the \mli{final scores}{'high-level embeddings' or 'logits' instead?} of each unimodal stream are combined \mli{at the end}{this is vague}. The combination could be by a weighted average of the scores~\cite{}, a bilinear product~\cite{}, or a more sophisticated rank minimization~\cite{} method. Another category of late fusion approaches is to use attention to pick the best expert for each input signal~\cite{jacobs1991adaptive}. The gated multimodal units~\cite{arevalo2017gated} extends this approach by enabling gating at intermediate feature levels. More recently, \mli{D. Hu and F. Nei}{inconsistent with citation style in use? I.e., no other citations specify the authors' names}~\cite{hu2019dense} proposed a dense multimodal early fusion network for hierarchical joint feature learning. Similar to~\cite{arevalo2017gated}, the dense fusion operator in~\cite{hu2019dense} also assumes identical spatial dimensions for different streams. Despite the similarity of these approaches to our work, their applicability is limited to certain layers where either spatial dimensions of multimodal features are identical or at the every end of the network where spatial dimensions are already aggregated. The squeeze operation in our method allows fusing modalities with different spatial dimensions at any level of the feature hierarchy.

In a related multimodal learning topic, called cross-modal learning, information from multiple modalities are used to improve the learning performance within any individual modality. It is assumed that data from all the modalities are present during training but the performance is tested on only one modality~\cite{ngiam2011multimodal}. MTUT~\cite{abavisani2019unimodal} uses spatiotemporal semantic alignment loss to improve the performance of each stream in gesture recognition. We believe cross-modal learning approaches are orthogonal to our work since the improved unimodal networks learned by this methods could be used as an initializer to our multistream network.

{\bf \noindent Multi-modal Action Recognition} Video~\cite{} and skeleton~\cite{} sensory modalities have been extensively used for the action recognition task. 
Another well-known work on video classification using deep neural networks shows superiority of slow fusion to the late fusion and early fusion of time-based, unimodal visual signals~\cite{karpathy2014large}.

{\bf \noindent Audio-visual speech enhancement} Work in audio-visual speech enhancement (AVSE) is strongly motivated by the cocktail party effect, which refers to humans' ability to selectively attend to auditory signals of interest within a noisy environment. Experiments in neuroscience have demonstrated that cross-modal integration of audio-visual signals may improve the perceptual quality of the targeted acoustic signal \cite{ghazanfar2003neuroperception, partan1999communication, rowe2002sound}. Inspired by the results from biological research, recent studies focus on augmenting audio only speech enhancement methods with visual information, such as lip movement. State-of-the-art results have been achieved by recent AV speech enhancement models that use deep neural networks \cite{afouras2018conversation, ephrat2018looking, afouras2019my, hou2018audio}. The predominant approach taken for AV fusion is late fusion \cite{katsaggelos2015audiovisual}, where the audio and visual information is processed separately then integrated at a singular point via channel-wise concatenation. 


{\bf \noindent Squeeze and Excitation (SE)
Network~\cite{Hu_2018_CVPR}} \mlic{This section doesn't fit well here at the end. he flow of the related works section can be improved by including this SEN part at the top where different mechanisms of fusion are introduced, and then end with the application subsections}
The proposed method can be seen as a generalization to the SE module, which is proposed for unimodal deep neural networks. The SE modules uses self excitation to adaptively recalibrate channel-wise feature activations. \mli{Our work adopts the SE module for multi-modal feature recalibrations}{This idea feels incomplete and the 2-3 sentences don't warrant a specific subsection. If we move this section as suggested in the comment above, we can just briefly touch upon it then go into the details in the section below.}.

==> backups/section_3.tex <==
\mli{\st{For simplicity suppose the input data has two modalities, a similar approach could be used for fusing more than two modalities. Assume there are two disjoint CNN streams to process each modality separately.}}{Rephrashing: In this section, we will discuss the case of two disjoint CNN streams, each of which independently processes a different modality of the input. The approach detailed here may be used for fusing arbitrarily many modalities.}. A MMTM receives the features of the modalities at some level in the networks' hierarchies, learns a global multimodal embedding from them, and uses this embedding to \mli{re-calibrate the input features.}{ensure consistency throughout text for 're-calibrate'; sometimes it's 'recalibrate' (without hyphen) and sometimes it's 're-calibrate' (with hyphen) -- I have changed all text to follow 'recalibrate' convention, but keep in mind for future text added.}

\mli{Let $\Ab \in \R^{N_1\times \dots \times N_K \times C}$ and $\Bb \in \R^{M_1\times \dots \times M_L \times C'}$\st{, the output of two convolution layers of each modality, be the input to the MMTM.}}{ represent the feature layers of the first and second CNN streams, respectively.} Here, $N_i$ and $M_i$ represent the spatial dimensions\footnote{In general, it is possible to have more than two (e.g. time dimension in 3D convolutions could be treated as a spatial dimension) or no (e.g. fully connected layers) spatial dimensions.}, and $C$ ($C'$) are feature-wise channels generated by applying $C$ ($C'$) convolution filters. Note that we do not assume the number of spatial dimensions \mli{{($L$ and $K$)}}{L and K are not well defined here. Does L correspond to stream 1 and K to stream 2? Or do L and K correspond to the 1st and 2nd spatial dimensions of N?} are equal between modalities.

{\bf \noindent Squeeze} The convolution layer features are information-limited by the size of the local receptive field are unable to exploit contextual information outside this region. As suggested by~\cite{Hu_2018_CVPR}, we first squeeze the spatial information into the channel descriptors by using a global average pooling over the spatial dimension of the input features:
\begin{align}
    S_\Ab(c) &= \frac{1}{\prod_{i=1}^{K} N_i}\sum_{n_1,\dots, n_K} \Ab(n_1, \dots, n_K, c) \\
    S_\Bb(c) &= \frac{1}{\prod_{i=1}^{L} M_i}\sum_{m_1,\dots, m_L} \Bb(m_1, \dots, m_L, c).
\end{align}
Note that while we use simple average pooling, more sophisticated pooling methods could be used at this step.

{\bf \noindent Multi-modal Excitation} The function of this unit is to generate the excitation signals, $E_A \in \R^C$ and $E_B \in \R^{C'}$, which can be used to recalibrate the input features, $\Ab$ and $\Bb$, by a simple gating mechanism:
\begin{align*}
    \tilde{\Ab} &= 2 \times \sigma(E_A) \odot \Ab \\
    \tilde{\Bb} &= 2 \times \sigma(E_B) \odot \Bb, \\
\end{align*}
where $\odot$ is the feature-wise product operation and $\sigma(.)$ is the sigmoid function. This allows the suppression or excitation of different filters in each stream. Note that the MMTM weights are regularized such that we can control the degree to which $E_A$ and $E_B$ remain close to zero. Thus, setting the regularization weight with the value of $2 \times \sigma(E_A)$ pushes the gating signal closer to $1$, limiting the amount that gating can change each stream signal. \mlic{Change phrasing above. Double check correctness.}

The gating signals should be a function of both inputs but also need to be predicted independently since each modality needs to change differently from each other. We achieve this by first predicting a joint representation from the squeezed signals
\begin{equation*}
Z = \Wb [S_\Ab, S_\Bb] + b,
\end{equation*}
and then predicting excitation signals for each modality through two independent fully-connected layers
\begin{equation*}
E_A = \Wb_A Z + b_A,\quad E_B = \Wb_B Z + b_B.
\end{equation*}
Here, $[\cdot, \cdot]$ represents the concatenation operation, $\Wb \in \R^{C_Z \times (C+C')}, \Wb_A \in \R^{C\times C_Z}, \Wb_B \in \R^{C'\times C_Z}$ are weights, and $b \in \R^{C_Z}, b_A \in \R^C, b_B \in \R^{C'}$ are the biases of the fully connected layers. As suggested by~\cite{Hu_2018_CVPR} we use $C_Z = (C+C')/4$ to limit the model capacity and increase the generalization power.

Learning the joint representation in this way allows the features of one modality to recalibrate the features of another modality. For instance, in gesture recognition when a gesture becomes blurry in RGB camera and more apparent in the depth, the depth stream could better excite more important filters in the RGB stream and suppress less useful one. This cross-modal recalibration affords more efficient processing in the RGB stream. Figure.~\ref{fig:mmtl} summarizes the overall architecture of the proposed MMTM.

\SKIP{\subsection{Transfer Madule Architecture}
We tried different module architecture for knowledge transfer in MMTM includes few convolution layers after concating the inputs, in order to do that the input to MMTM from each modal should have similar dimension. This limited our use case to the modalities which are spatially related to each other  such as RGB and Depth or Optical Flow. Other option would be fully connected layers, this is doable by arbitrary inputs but could be huge for a early and mid layers in networks. Finally motivated by squeeze and extraction idea \cite{Hu_2018_CVPR} we apply an average pooling on inputs to squeeze the MMTM inputs. This allow us to have arbitary input shapes to MMTM. Figure.~\ref{fig:mmtl} shows proposed architecture for MMTM for three inputs for visualization purposes while it could be for $N$ inputs. As we discussed, first the inputs are squeezed by an average pooling layer to generate $N$ vector with size of $b \times 1 \times 1 \times 1 \times c_i$ where $b$ and $c_i$ are batch size and channel dimension for modality $i$  then the channels are concatenated to generate an output of $b\times1\times 1\times1\times \sum c_i$. Then a fully connected layer with Relu activation transfer it to $b \times 1 \times 1 \times 1 \times \dfrac{\sum c_i}{4}$. Finally for each modality $i$ another fully connected with sigmoid activation transfer it to $b \times 1 \times 1 \times 1 \times \sum c_i$. Finally the output of MMTM is gated to the output of last layer to generate the input for next layer for each modality.

\subsection{Number of parameter and operation}

The average pooling at the beginning of MMTM reduce the number of operation for it significantly but the number of parameter to be learn is fixed. For fist fully connection layer there are $\dfrac{(\sum c_i)^2}{4}$ parameters and for second convolution layer there are similar number of parameters. Since there is no other parameters the total number of parameters for MMLT would be $\dfrac{(\sum c_i)^2}{2}$. Since all the operation applied to squeezed feature vector the number of multiplication is also $\dfrac{(\sum c_i)^2}{2}$ plus $\sum (t_i \times w_i \times h_i \times c_i)$ for gating. Although the number of parameters for a single MMTM is comparable with convolution layers $\sum (k_i^3 \times d_i \times c_i)$ assuming $d_i$ is the input size to convolution layer and kernel size is $[k,k,k]$. But the number of operation is much much less compared to $\sum (k_i^3 \times t_i \times w_i \times h_i \times d_i \times c_i)$. Let's assume number of channel is always $c$ and all other dimensions are equal to $w$ so the ratio of number of parameters of MMTM to a $N$ convolution of current layer is $\dfrac{N}{2k^3}$ and the ratio of number of multiplications of MMTM to a $N$ convolution of current layer is approximately $\dfrac{N}{2k^3w^3}$. As we expect the number of parameters is comparable while the number of operation is negligible. Although in practice each layer includes multiple number of convolutions such as inception module or resnet blocks.}  

==> more_shortcuts.tex <==

\usepackage{microtype} % not sure whether we use this or not
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{multirow}
\usepackage{caption}

\graphicspath{ {../figures/} }

\def\d{\text{\normalfont d}}

% whether to inlcude proofs
\newif\ifLONG
%\LONGtrue
\LONGfalse
\ifLONG % just print the proof on spot in the long version
\renewenvironment{proofatend}{\begin{proof}}{\end{proof}}
\fi


% Necessary in order to have theorems, propositions, and lemmas use the same counter
\theoremstyle{plain}
\newtheorem{prop}[theorem]{\bf Proposition}
%\newtheorem{lem}[theorem]{\bf Lemma}

% For restating the theorems in the appendix
%\newtheorem*{theorem*}{\bf Theorem}
%\newtheorem*{prop*}{\bf Proposition}
%\newtheorem*{lem*}{\bf Lemma}




==> skip.tex <==
\SKIP{
\begin{figure}
    %\vspace{-.4in}
	\begin{center}
		\includegraphics[width=1\linewidth]{i3d_mmtl.pdf}
	\end{center}
	\vspace{-.1in}
	\caption{\mlic{Still shows MMTL - needs to be update to MMTM}Proposed fusion network for video classification includes last 6 layers of inflated inception3D and MMTM. This is the fusion for three modality of RGB, depth and optical flow. Inc. denote inception module from \cite{carreira2017quo}  }
	\label{fig:i3d_mmtl}
	\vspace{-0.1in}
\end{figure}
}


\SKIP{
\subsection{Scene Recognition}

SUN RGB-D~\cite{song2015sun}: The dataset contains 10,335 RGB-D images from NYU depth v2 data set~\cite{silberman2012indoor}, Berkeley B3DO data set~\cite{janoch2013category}, and SUN3D data set~\cite{xiao2013sun3d}.  We follow the experiment settings stated in ~\cite{song2015sun} and only keep categories with more than 80 images which includes 19 categories. Using the publicly available split, there are in total 4,845 images for training and 4,659 images for testing. We report the means of diagonal values of the confusion matrices, which are the average precisions over all scene classes similar to \cite{wang2016modality}. 


\begin{table}[t]
\begin{center}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{ l c c}
%\hlineB{3}
%\cline{3-7}
%\cline{2-3} 
 Method   & Fused modalities & Accuracy\\% & Fusion (RGB-D)\\%   & Avg.          $\pm$  std.      \\

\hline
~\cite{song2015sun} &	RGB+Depth & 			 \\
~\cite{liao2016understand} &	RGB+Depth & 			 \\
~\cite{wang2016modality} &	RGB+Depth 	& 			 \\
~\cite{song2017combining} &	RGB+Depth 	& 			 \\
MMTM~(ours) &	RGB+Depth	& 	\bf{}		 \\
\hline
\end{tabular}%}
%\vspace{2.5mm}
\caption{Accuracies of different multimodal fusion scene recognition methods on the SUN RGB-D dataset~\cite{song2015sun}. The top performer is denoted by boldface.} \label{tbl:multi_sun}
\end{center}
\vspace{-2.5mm}
\end{table}
}
